Power Deposition on Tokamak Plasma-Facing Components

The SMARDDA software library is used to model plasma interaction with complex engineered surfaces. A simple flux-tube model of power deposition necessitates the following of magnetic fieldlines until they meet geometry taken from a CAD (Computer Aided Design) database. Application is made to 1) models of ITER tokamak limiter geometry and 2) MASTU tokamak divertor designs, illustrating the accuracy and effectiveness of SMARDDA, even in the presence of significant nonaxisymmetric ripple field. SMARDDA's ability to exchange data with CAD databases and its speed of execution also give it the potential for use directly in the design of tokamak plasma facing components.

==> details.tex <==
%\subsection{Particle Pushing by SMARDDA}
The SMARDDA algorithm is encapsulated as a function which takes
a straight particle track,
specified by its start and end points, and determine whether
it intersects any part of the geometry. If so, it returns
the first point of intersection.
The track is defined by two arguments of type {\tt posnode},
a type which consists of  a position vector and the identifier of the 
deepest corresponding node in the octree. Frequently, the node
of the start position is known as the result of a previous
calculation, if not, as occurs typically on the first step,
it is calculated by binary look-up in the octree. The second argument
will acquire a nodal value only upon exit, corresponding to
the end of the track. Its position vector will be changed from
the input value only if the track intersects the geometry as
signalled by the return of another, the last, function argument.
%Other arguments are the octree data structure associated with the list of geometrical
%objects defining the constraints on particle motion, typically
%a triangular meshing of the duct walls, and the list itself. Internally, there are
%logical parameters which can be set so the routine can handle
%unquantised positions and/or take larger steps through the
%geometry.

The function uses the same-cell test of \Sec{samec}
as a preliminary check. This is efficient when
particle trajectories are short.
%whether the first and second positions
%are in the same nodes or lie in nodes that share a common face.  Here `node' is used
%as a synonym for voxel, the volume of quantised space corresponding to
%the node of the octree. This preliminary checking is efficient when
For longer tracks, the
particle advance is controlled by a loop in the first coordinate~$x_1$.
For reasons which will become apparent,
particle track is started from a virtual origin,
viz. an integer (quantised) position in the first coordinate, either the largest
integer less than the start position if the motion is forwards,
or the smallest integer greater than the start position if motion
is backwards, see the illustration in \Fig{vpos}.

%Note that these position vectors are referred
%to as `quantised', even when they are expressed as real numbers with
%non-vanishing fractional part.
%Ideally, the longer trajectories would be specified by a start point
%and a direction. To use the interface to the SMARDDA algorithm
%provided, it is necessary to specify an end-point within the meshed
%volume. In general, this might be difficult to arrange. However, for a
%duct, neutral trajectories can be arranged to terminate on a plane
%slightly beyond the end of the duct, say distance $L_{term}$ from the
%launch-point, then the maximum deviation in the plane from
%the duct axis will be $L_{term}/\cos{(\theta)}$. If a triangle pair
%is arranged so as to span the rectangle with
%corners~$(\pm L'_{term}/\cos{(\theta)},\pm L'_{term}/\cos{(\theta)},L'_{term})$ then
%all end-points on the terminating plane~$z=L_{term}=L'_{term}-\Delta$
%will lie in the computational volume.
\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{vpos}\\
\caption{The track projected on the $x_1 x_2$-plane, with integer
coordinate values shown as a grid.
The track is defined by the start
point~$o$ and the end point~$n$, joined by an arrow
to indicate direction of travel. The virtual origin~$v$
is constructed as indicated to have an integer~$x_1$ coordinate.}
\label{fig:vpos}
\end{figure}

In the DDA applied conventionally to a SEADS, each
subsequent increment of the integer loop counter gives
a position in a different cell along the track.
Supposing that lateral motion of the particle relative
to the first coordinate direction is negligible,
the first position coordinate is incremented by one
when motion is forwards, or decremented by unity when motion is backwards. 
First, the track is tested against objects
in the cell indexed by the octree node corresponding to the start position,
and if there is a collision ``in the node", the track
terminates at the intersection point. If there is no collision, there
is a same-cell test of the new position and the end-point of the track.
If this is true, the loop terminates,
otherwise the position is updated and the loop continues in
a new cell with collision tests etc.

The advance along the track is complicated in higher dimensions
because the track may enter new nodes as a result of its motion
in the other coordinates. It is efficient to arrange so that the 
particle moves farthest in the direction of the first coordinate, by
relabelling if necessary. The other two coordinates may be chosen purely
so that the relabelled coordinates~$(x_1,x_2,x_3)$ form a right-handed set. 
In the resulting (quantised) coordinate system, the vector of
advance is $(\alpha_1,\alpha_2,\alpha_3)$ where $\alpha_1=\pm 1$,
$|\alpha_2|<1$ and $|\alpha_3|<1$.
In outline, coordinate~$x_2$ is incremented by~$\alpha_2$ to see
whether this point lies in a new node, then 
coordinate~$x_3$ is incremented by~$\alpha_3$ and this point
tested, and finally
all three coordinates are updated, and the new point tested.
The latter point now on the track, is then updated like the first virtual point,
and so on.

In detail, consider first the $x_2$~update.
There is a quick test as to 
whether the integer part of $x_2$ has changed,
%(a test which could in fact
%be omitted depending on the relative expense of conditional operations),
then if so, a test whether the new~$x_2$ position, shown as
point~$2':(x_1,x_2+\alpha_2,x_3)$ 
in \Fig{detupd}, lies in the current node. If $2'$ is found to 
lie in a new node, the objects in that node are tested for
collision with the track, and if no collision is found, the code proceeds. The
coordinate~$x_3$ is updated to give the
point~$3':(x_1,x_2,x_3+\alpha_3)$, which of course may lie in a new node,
and if so, the node is tested for collisions in the same way. There
is the additional complication that the
point~$4':(x_1,x_2+\alpha_2,x_3+\alpha_3)$ may lie in a node
different to that of either of the points~$2'$ and~$3'$.
If so, a further test for collision is performed in this third node.
However, this is the maximum number of nodes that
need testing between updates of~$x_1$.
%this is strictly only required for multi-dimensional motions)
%Note that the asymmetry in the particle motion caused by the
%restriction of $x_1$ to integer values means that a maximum of
%three nodes


Moreover, and distinguishing
the SMARDDA algorithm from the DDA variant above,
the increment in unity of the
position~$x_1$ is replaceable by increments which
could be as large as $2$,~$4$, $8$~or more.
%of the size of the deepest local cuboid of the octree, ie.\
The idea is to jump along the track as far forwards in the current
cell as possible, to an integer point $x_1$, such that the
next integer increment of $x_1$ will produce a point in a new cell,
possibly laterally displaced.

The underlying mathematics are as follows. For DDA it is anyway convenient
to introduce binary markers $d_j$ which are unity for forwards
motion in direction~$j$ and zero for backwards. Supposed the quantised size of
the cell is $2^{\ell_k}$ where $k$~labels the octree level, then
if $o_j$ are the coordinates of the current cell's origin,
the path increment~$\Delta$ can be calculated using
\begin{equation}
\Delta_j=\left(o_j+ ISHFT(d_j, \ell_k) -x_j\right)/\alpha_j,\;\;\;j=1,2,3
\end{equation}
as
\begin{equation}
\Delta= INT\left(\min{\{\Delta_1, \Delta_2, \Delta_3, |x^E_1-o_1|,
ISHFT(1, \ell_k)-1\}}\right)
\end{equation}
(The last term corresponds to a displacement limited by the cell size,
and the second-last
accounts for a track ending at~${\bf x}^E$.)
One step of the DDA algorithm can then be applied as though beginning from
the position
\begin{equation}
{\bf x}'=(o_1,x_2,x_3)+(\alpha_1,\alpha_2,\alpha_3)\Delta
\end{equation}
but note the need for special treatment at the track end-point.
The concept of virtual origin is important here, in that
the track can be tested in sections defined by a sequence of
virtual origins each corresponding to an integer value of~$x_1$.

\begin{figure}
\centering
\includegraphics[width=2.75in]{detupd}\\
\caption{Segment of track projected on the $x_2 x_3$-plane, with 
boundaries of the smallest local cells shown. As the track is
incremented by a unit quantity in the $x_1$~direction, it moves
from the point~$o$ in the lower right-hand node to the point~$4'$
in the upper-left by the vector displacement~$(\alpha_2,\alpha_3)$. The nodes containing points~$2'$ and~$3'$ are
tested for colliding objects, the former unnecessarily in this instance.}
\label{fig:detupd}
\end{figure}


%For speed, the node corresponding to a position is never
%calculated by look-up from the root of the octree, except possibly on the
%first step. There is always a test using the IEOR function
%as described in \Sec{PT}, to see whether one position
%lies in the same node as another position in a known node,
%usually close by on the particle track. The known node can thus be used as a 
%starting point for locating the node of the new position.
%For further speed, there is an option controlled by
%a constant parameter variable to move multiple steps
%in~$x_1$, with number of steps only limited so that the first
%coordinate on the track still lies in the node.

Last details are that the testing of the track for collisions is
performed using Badouel's algorithm~\cite{Ba90Effi}, modified to take
into account finite precision computer arithmetic as in ref~\cite{Ha07Effi}.
Where the point of intersection of the track with the object face is
needed, eg.\ for diagnostic purposes, it is computed as in the second step of 
Badouel's algorithm~\cite{Ba90Effi,Ha07Effi}.

%The code remembers to check whether the track 
%intersects more than one object in the node, and selects
%the nearest to the start point. It also checks that the intersection does in fact
%take place in the node.

%\end{document}

